A CFL-type Condition and Theoretical Insights for Discrete-Time Sparse Full-Order Model Inference

In this work, we investigate the data-driven inference of a discrete-time dynamical system via a sparse Full-Order Model (sFOM). We first formulate the involved Least Squares (LS) problem and discuss the need for regularization, indicating a connection between the typically employed $l_2$ regularization and the stability of the inferred discrete-time sFOM. We then provide theoretical insights considering the consistency and stability properties of the inferred numerical schemes that form the sFOM and exemplify them via illustrative, 1D test cases of linear diffusion and linear advection. For linear advection, we analytically derive a "sampling CFL" condition, which dictates a bound for the ratio of spatial and temporal discretization steps in the training data that ensures stability of the inferred sFOM. Finally, we investigate the sFOM inference for two nonlinear problems, namely a 2D Burgers' test case and the incompressible flow in an oscillating lid driven cavity, and draw connections between the theoretical findings and the properties of the inferred, nonlinear sFOMs.

==> stashed.tex <==
Finally, in \Cref{regularization}, we indicated a connection between the $L_2$ regularization in \eqref{LS_reg} with the stability of the inferred discrete-time sFOM, via the Gershgorin disk theorem \eqref{GerSt}. For a 2-point stencil, i.e., $Q_i=\{ i, \;i+1 \}$, we derive the analytical solution of \eqref{LS_reg} using the approximations in \eqref{taylor_data} and \eqref{taylor_future}. Following the argumentation in \Cref{CFL_section}, the analytical solution for \eqref{LS_reg} reads as

\begin{multline}
\label{anal_reg}
{\bm{\beta}_i}_j = \frac{\left( K_{1_i}+\eta_i \Delta x^{-2} (a+\Delta t g) \right) + j (K_{2_i}+\eta_i \Delta x^{-2}( a+\Delta x d + \Delta t g + \Delta x \Delta t e) }{(ab-d^2) + \eta_i(2a \Delta x^{-2}+2d\Delta x^{-1}+b)}, \quad j \in \{0,1\}
\end{multline}

For $\eta_i=0$, we obtain \eqref{approxD} (for the 2-point stencil), since it corresponds to the non-regularized LS problem \eqref{LSform}. An interesting result is obtained by considering the Gershgorin disk radius of \eqref{approxD} and\eqref{anal_reg}. Assuming that $\|{\bm{\beta}_i}_j\|={\bm{\beta}_i}_j$, we obtain

\begin{equation}
\| \bm{\beta}_i(\eta_i>0) \|_1=\frac{1+\eta_i \frac{2a}{K_{1_i}+K_{2_i}}{} 
\end{equation}
